Extension of Minimax for Algorithmic Lower Bounds

This paper considers the use of Yao's Minimax Theorem in robust algorithm design, e.g., for online algorithms, where the algorithm designer aims to minimize the ratio of the algorithm's performance to the optimal performance. When applying Minimax, the objective becomes the expectation of these ratios. The main result of the paper is that it is equally valid for the objective (after applying Minimax) to be the ratio of the expectations.

==> sim_alg_robust.tex <==


\section{Minimax in Robust Algorithm Design}
\label{s:robustalgs}

Robust algorithm design fits directly into the Minimax framework.  An abstract definition of an arbitrary {\em algorithm problem setting} $\algprob=(\algspace, $ defines an algorithm space $\algspace$ which is a set of algorithms $\algo=\omega$: $$\algspace = \{\spaceomi[a]~|~\text{paremeters}~\spaceomi[a]~\text{describe a legal algorithm} \}$$


In this setting, the ratio explicitly becomes:

(a) a {\em raw designer's performance} $\algo:\despace \times \stspace \rightarrow \reals_+$ {\em benchmark} function which is a pure measure of the state $\spaceomi[2]$


We restate our main result as it applies to the general setting of robust algorithm design.  Practically, we note that this lower bound is only an abstraction because we don't say anything about how to optimize the algorithm $\algo$.

\ajc{the immediately preceding question here is copied from original blends manuscript; the next equation should fix $\algo(\cdot)$ in the denominator, and be written in a way that benchmark is not specified -- it may later be set to either the PF or PI benchmark}



